Revisit Few-shot Intent Classification with PLMs: Direct Fine-tuning vs. Continual Pre-training

We consider the task of few-shot intent detection, which involves training a deep learning model to classify utterances based on their underlying intents using only a small amount of labeled data. The current approach to address this problem is through continual pre-training, i.e., fine-tuning pre-trained language models (PLMs) on external resources (e.g., conversational corpora, public intent detection datasets, or natural language understanding datasets) before using them as utterance encoders for training an intent classifier. In this paper, we show that continual pre-training may not be essential, since the overfitting problem of PLMs on this task may not be as serious as expected. Specifically, we find that directly fine-tuning PLMs on only a handful of labeled examples already yields decent results compared to methods that employ continual pre-training, and the performance gap diminishes rapidly as the number of labeled data increases. To maximize the utilization of the limited available data, we propose a context augmentation method and leverage sequential self-distillation to boost performance. Comprehensive experiments on real-world benchmarks show that given only two or more labeled samples per class, direct fine-tuning outperforms many strong baselines that utilize external data sources for continual pre-training. The code can be found at https://github.com/hdzhang-code/DFTPlus.

==> latex_figures/latex_figures_analysis_acc_vs_GPT3_temperature.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.45]{resources/analysis_acc_vs_GPT3_temperature_banking77_HWU64.png}
    \caption{The impact of GPT-3 temperature on model performance. The context size is $50$ per label.}
    \label{figure: acc_vs_GPT3_temperature}
\end{figure}

==> latex_figures/latex_figures_analysis_acc_vs_context_size.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.45]{resources/analysis_acc_vs_context_size_banking77_hwu64.png}
    \caption{The impact of augmented context size on model performance. When the size is $0$, only the utterances in the small training dataset $\mathcal{D}$ is used for MLM.}
    \label{figure: acc_vs_context_size}
\end{figure}

==> latex_figures/latex_figures_analysis_acc_vs_self_distillation_generations.tex <==


\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.45]{resources/analysis_acc_vs_self_distillation_generations_banking77_hwu64.png}
    \caption{Model performance at different self-distillation generations.}
    \label{figure: acc_vs_self_distillation_generations}
\end{figure}

==> latex_figures/latex_figures_analysis_acc_vs_self_distillation_temperature.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.45]{resources/analysis_acc_vs_GPT3_temperature_banking77_HWU64.png}
    \caption{The impact of the temperature of sequential self-distillation on model performance.}
    \label{figure: acc_vs_self_distillation_temperature}
\end{figure}

==> latex_figures/latex_figures_analysis_hyper_contextual_aug.tex <==
\begin{figure}[h]
\centering
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[scale=0.24]{resources/analysis_acc_vs_context_size_banking77_hwu64_smallFig.png}
        \caption{Augmented context size.}
        \label{figure: hyper-parameters, contextual augmentation, augmented context size}
    \end{subfigure}
     % \hspace{6mm}
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        % \includegraphics[scale=0.45]{resources/acc_isotropy.png}
        \includegraphics[scale=0.24]{resources/analysis_acc_vs_GPT3_temperature_banking77_HWU64_smallFig.png}
        \caption{GPT-J temperature.}
        \label{figure: hyper-parameters, contextual augmentation, GPT-J temperature}
    \end{subfigure}
\caption{Impact of augmented context hyper-parameters with experiments on $5$-shot tasks. When the context size is $0$, only the few utterances is used for MLM. CA denotes context augmentation.}
\label{figure: hyper-parameters, contextual augmentation}
\end{figure}

==> latex_figures/latex_figures_analysis_hyper_knowledge_distillation.tex <==
\begin{figure}[h]
\centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[scale=0.24]{resources/analysis_acc_vs_self_distillation_generations_banking77_hwu64_smallFig.png}
        \caption{Generations.}
        \label{figure: hyper-parameters, self-distillation, generations}
    \end{subfigure}
     % \hspace{6mm}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[scale=0.24]{resources/analysis_acc_vs_self_distillation_temperature_banking77_hwu64_smallFig.png}
        \caption{Temperature.}
        \label{figure: hyper-parameters, self-distillation, temperature}
    \end{subfigure}
\caption{Impact of knowledge-distillation hyper-parameters on: generations and temperature $t$. The data is collected on $5$-shot tasks.}
\label{figure: hyper-parameters, self-distillation}
\end{figure}

==> latex_figures/latex_figures_main_result_acc_vs_shot_banking_backup.tex <==
\begin{figure}[h]
\centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[scale=0.40]{resources/main_result_ac_vs_shot_bert_banking_simple.png}
        \caption{BERT-based experiments.}
        \label{figure: main_result_acc_vs_shot_bert}
    \end{subfigure}
     % \hspace{6mm}
     \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        % \includegraphics[scale=0.45]{resources/acc_isotropy.png}
        \includegraphics[scale=0.40]{resources/main_result_ac_vs_shot_roberta_banking_simple.png}
        \caption{RoBERTa-based experiments.}
        \label{figure: main_result_acc_vs_shot_roberta}
    \end{subfigure}    
\caption{Impact of the size of labeled data on performance. The data is collected on BANKING77. Top-2 baselines are presented.}
\label{figure: main_result_acc_vs_shot}
\end{figure}

==> latex_figures/latex_figures_main_result_acc_vs_shot_banking_small.tex <==
\begin{figure}[h]
\centering
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[scale=0.24]{resources/main_result_ac_vs_shot_bert_banking_simple_smallFig.png}
        \caption{BERT-based.}
        \label{figure: main_result_acc_vs_shot_bert}
    \end{subfigure}
     % \hspace{6mm}
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        % \includegraphics[scale=0.45]{resources/acc_isotropy.png}
        \includegraphics[scale=0.24]{resources/main_result_ac_vs_shot_roberta_banking_simple_smallFig.png}
        \caption{RoBERTa-based.}
        \label{figure: main_result_acc_vs_shot_roberta}
    \end{subfigure}    
\caption{Impact of the size of labeled data on performance. The data is collected on BANKING77. Top-2 baselines are presented.}
\label{figure: main_result_acc_vs_shot}
\end{figure}

==> latex_figures/latex_figures_pilot_study_overfit_v2.tex <==

\begin{figure}[h]
\centering
    \includegraphics[width=0.47\textwidth]{resources/shot15.png}
    \caption{The accuracy of the model on test partition during few-shot fine-tuning of BERT. The fine-tuning is robust to overfitting.}
    \label{figure: overfit_analysis}
\end{figure}

% \includegraphics[width=0.5\textwidth]{my-uploaded-figure.png}

==> latex_tables/analysis_GPT_examples_backup.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{p{5.0cm}p{5.0cm}p{5.0cm}}
\toprule
Input & Good & Bad \\
\midrule
% ``pending transfer''
%``How long is a \textcolor{green}{transfer} in the \textcolor{green}{pending} status?'', ``Why is there a \textcolor{green}{pending} time on my \textcolor{green}{transfer}?'', ``The \textcolor{green}{transfer} was accepted but now it is \textcolor{green}{stuck on pending} when will it go through?'', ``So my \textcolor{green}{transfer} is showing as \textcolor{green}{pending} when will it actually \textcolor{green}{go through}?'', ``How long does it take for \textcolor{green}{pending transfer transactions} to post?'' ``'' 
%&  
%``What is the status of my brothers \textcolor{green}{pending transfer}?'', ``i need to see if my \textcolor{green}{money} has been posted with the \textcolor{green}{transfer} yet'', ``why is my \textcolor{green}{transfer} name and status not changing'', ``my \textcolor{orange}{order} was approved but is \textcolor{green}{stuck in a pending status} and i want to know why'', ``'what is the \textcolor{orange}{difference} between \textcolor{green}{pending} and \textcolor{orange}{incomplete}''
%& 
% ``answer to my above question'' \\
% \midrule
``Is there a reason why my \textcolor{green}{card was declined} when I attempted to \textcolor{green}{withdraw money}?'', ``How come I can not \textcolor{green}{get money} at the \textcolor{green}{ATM}?'', ``Why can not I \textcolor{green}{withdraw cash} from this \textcolor{green}{ATM}?'', ``Why will not the \textcolor{green}{ATM} give me \textcolor{green}{cash}?'', ``This morning, I wanted to \textcolor{green}{make a withdrawal} before work but my \textcolor{green}{card was declined}, please double check it for me as this is the first time it \textcolor{green}{was declined}.''
&
``\textcolor{green}{ATM} will not let me \textcolor{green}{withdraw my money} my card as \textcolor{green}{refused} please help'', ``I \textcolor{green}{withdrew} less than I expected from the \textcolor{green}{ATM} on monday'', ``My \textcolor{orange}{wallet was stolen} but my \textcolor{green}{ATM card} was within safely'', ``I \textcolor{orange}{spent a fortune} last week and have none left on my \textcolor{green}{card} can you reverse \textcolor{green}{refund the fees}'',``\textcolor{orange}{Please give me the code} that I can use in the \textcolor{green}{ATM} for my face to \textcolor{green}{use my card}''
& 
``Why did my card never get a their villages and journey?'', ``An autofill took place but there was nothing to approve.'',  ``Can I get one form my card after I have made a ctifre?'', ``Family needs money for the holidays they said they can not make it I hope you can help even if it is not much.'' \\
\midrule
``Please \textcolor{green}{order take} from Jasons Deli.'', ``Can you please \textcolor{green}{order some food} for me?'', ``Can you look up Chinese \textcolor{green}{takeout} near here?'', ``Can i \textcolor{green}{order takeaway} from Spanish place?'', ``Find and \textcolor{green}{order} rasgulla of janta sweet home pvt ltd.''
&
``I need to \textcolor{green}{get some gluten free cookies} for my daughter'', ``Can you do ticket counter \textcolor{green}{take away}'', ``How can I \textcolor{green}{order Chinese food}'', ``\textcolor{orange}{Delivery service} please \textcolor{green}{order some takeaway} jahdi'', ``\textcolor{green}{Order} beef kasundi bewa rasgulla and dosa \textcolor{orange}{will be ready} in 10 mins''
&
``Please make some reservation if you want booking on myhotelcom'', ``Drive take from a taxi'', ``Warehouse 26723'', ``Please make some reservation if you want booking on  myhotelcom''
\\
% \midrule
% ``what are symptoms'', 'what should i check to see if i \textcolor{green}{have the disease}', 'are the \textcolor{green}{symptoms} of covid 19 similar to allergies', 'how long should i wait to get help if i show \textcolor{green}{signs of corona}', 'does \textcolor{green}{coughing up} mean i have the corona', 'can you please tell me the \textcolor{green}{symptoms} of coronavirus'
% &
% ``why did her husband bring a \textcolor{green}{corona} patient to the \textcolor{orange}{hospital}'', ``what should be done to \textcolor{orange}{prevent spreading} \textcolor{green}{corona virus}'', ``i feel more \textcolor{orange}{headaches} but the \textcolor{orange}{headaches} do not leave my eyes'', ``if i show \textcolor{green}{symptoms of the corona} should i shake my hands with the \textcolor{orange}{doctor}'', ``should i postpone my \textcolor{orange}{surgery} when i \textcolor{green}{have coughing}''
% &
% ``what is confirmed at this stage'', ``'what is the difference between methane poisoning and cyanide poisoning'', ``my pregnant adult friend has had but it cleaorange up''
% \\
\bottomrule
\end{tabular}
\caption{Utterances generated by GPT-J. The first row is for label ``Declined Cash Withdrawal'' from BANKING77. The second row is for label ``Takeaway Order'' from HWU64. Good examples are semantically relevant to the input data, while bad examples are irrelevant. Both \textcolor{green}{green} and \textcolor{orange}{orange} words are highlighted to show the semantic relevance, but orange words deviate the sentence from the original label.}
\label{table: analysis_examples_GPT3}
\end{table*}

==> latex_tables/analysis_ablation.tex <==
\begin{table}[h]
%% local redefinitions
% \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
% \renewrobustcmd{\boldmath}{}
\centering
\small
\begin{tabular}{ccccc}
\toprule
FT & MLM & CA & SSD & val. &  \\
\midrule
\checkmark &  &  &  & 80.38\tiny(.35) \\
% \midrule
\checkmark &  &  & \checkmark  & 82.38\tiny{(.38)} \\
\midrule
\checkmark & \checkmark &  &  & 83.45\tiny{(.35)} \\
\checkmark & \checkmark &  & \checkmark  & \textbf{84.18\tiny{(.28)}} \\
\midrule
\checkmark &  &  \checkmark &  & 83.94\tiny{(.45)} \\
\checkmark & &  \checkmark  & \checkmark  & \textbf{84.67\tiny{(.51)}} \\
\midrule
\checkmark & \checkmark  &  \checkmark &  & 85.21\tiny{(.58)} \\
\checkmark & \checkmark  &  \checkmark  & \checkmark  & \textbf{85.64\tiny{(.41)}} \\
%\midrule
\bottomrule
\end{tabular}
% \caption{Main results for $5$-way tasks. $\ssymbol{5}$ stands for results from the original paper. $\ssymbol{2}$ represents models that employ Roberta.}
\caption{
%The complementarity of the proposed methods and batch normalization. 
Effect of combining batch normalization and our method. The experiments are conducted with BERT and evaluated on $5$-way $2$-shot tasks. SPT denotes supervised pre-training. BN denotes batch normalization.}
\label{table: analysis_ablation}
\end{table}

==> latex_tables/analysis_context_aug_versus_data_aug.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{p{3.65cm}>{\centering\arraybackslash}p{1.5cm}c}
\toprule
Method & BANKING77 & HWU64 \\
\midrule
DFT        & 69.01\tiny(1.54)   &  75.07\tiny(.53) \\
\midrule
EDA~\cite{wei-zou-2019-eda}        & 68.81\tiny(1.97) & 74.68\tiny(.81)  \\
BT~\cite{edunov-etal-2018-understanding}         & 69.65\tiny(1.39)  & 74.15\tiny(.84) \\  
PromDA~\cite{wang-etal-2022-promda}     & 69.84\tiny(1.10) & 75.78\tiny(.64)  \\ 
SuperGen~\cite{meng2022generating}   & 64.83\tiny(1.06) & 69.52\tiny(0.56)  \\ 
GPT-J-DA~\cite{sahu-etal-2022-data}      & 71.84\tiny(1.41) & 70.72\tiny(.78)  \\ 
\midrule
Context augmentation & \textbf{72.23\tiny(1.80)} & \textbf{76.73\tiny(1.05)} \\
\bottomrule
\end{tabular}
\caption{Comparison of context augmentation against data augmentation based on BERT with 5-shot tasks.}
\label{analysis_context_aug_versus_data_aug}
\end{table} 

==> latex_tables/analysis_context_aug_versus_data_aug_full_backup.tex <==
\begin{table*}[t]
%% local redefinitions
% \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
% \renewrobustcmd{\boldmath}{}
\begin{subtable}{1.0\textwidth}
\centering
\small
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & 
\multicolumn{2}{c}{BANKING77} &
\multicolumn{2}{c}{HINT3} &
\multicolumn{2}{c}{HWU64} &
\multicolumn{2}{c}{MCID}  
\\
\cmidrule(lr){2-3}  \cmidrule(lr){4-5}  \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& 5-shot & 10-shot & 5-shot & 10-shot & 5-shot & 10-shot & 5-shot & 10-shot\\
\midrule
% ChildTune & xx & xx & xx  & xx & xx  & xx  & xx  & xx  \\
% NoisyTune & xx & xx & xx  & xx & xx  & xx  & xx  & xx  \\
DFT & 69.01\tiny(1.54) & 78.92\tiny(1.69) &  60.65\tiny(1.60)  & 66.36\tiny(3.48) & 75.07\tiny(.53)  & 82.38\tiny(1.49)  & 72.32\tiny(1.80)  & 80.53\tiny(1.15)  \\
\midrule
EDA & 68.81\tiny(1.97) & 72.97\tiny(.94) & 60.50\tiny(3.06) & 59.94\tiny(1.10) & 74.68\tiny(.81)  & 72.76\tiny(5.16)  & 73.10\tiny(.64)  & 80.99\tiny(.16)  \\
BT & 69.65\tiny(1.39) & 78.42\tiny(.83) & 60.50\tiny(1.40)  & 66.33\tiny(2.69) & 74.15\tiny(.84)  & 79.12\tiny(1.65)  & 75.15\tiny(2.04)  & 81.36\tiny(1.6)  \\
PrompDA & 70.36\tiny(1.85) & 78.85\tiny(1.56) & 58.08\tiny(4.98)  & 64.56\tiny(3.64) & 69.86\tiny(4.27)  & 74.87\tiny(3.02)  & 70.80\tiny(3.16)  & 78.60\tiny(1.49)  \\
SuperGen & 70.36\tiny(1.85) & 78.85\tiny(1.56) & 58.08\tiny(4.98)  & 64.56\tiny(3.64) & 69.86\tiny(4.27)  & 74.87\tiny(3.02)  & 70.80\tiny(3.16)  & 78.60\tiny(1.49)  \\
GPT-J & 71.84\tiny(1.41) & 78.34\tiny(.87) & 60.24\tiny(.83) & 67.40\tiny(2.41) & 70.72\tiny(.78) & 76.66\tiny(1.3)   & 73.92\tiny(2.77) & 78.77\tiny(2.39)  \\
\midrule
CA & \textbf{72.23\tiny{(1.80)}} & \textbf{82.33\tiny{(.72)}} & 60.53\tiny{(2.73)} & \textbf{70.36\tiny{(1.90)}} &  76.73\tiny{(1.05)} & 82.61\tiny{(.23)} & 77.45\tiny{(1.66)} & 81.27\tiny{(1.41)} \\
\bottomrule
\end{tabular}
\caption{BERT-based evaluation results.}
\label{table: table: analysis_context_aug_versus_data_aug_full: subtable, bert}
\end{subtable}
% \\
\newline
% \newline
\begin{subtable}{1.0\textwidth}
\centering
\small
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & 
\multicolumn{2}{c}{BANKING77} &
\multicolumn{2}{c}{HINT3} &
\multicolumn{2}{c}{HWU64} &
\multicolumn{2}{c}{MCID}  
\\
\cmidrule(lr){2-3}  \cmidrule(lr){4-5}  \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& 5-shot & 10-shot & 5-shot & 10-shot & 5-shot & 10-shot & 5-shot & 10-shot\\
\midrule
% ChildTune & xx & xx & xx  & xx & xx  & xx  & xx  & xx  \\
% NoisyTune & xx & xx & xx  & xx & xx  & xx  & xx  & xx  \\
DFT & 76.11\tiny(1.16) & 84.77\tiny(.43) & 61.39\tiny(1.51)  & 68.40\tiny(1.21) & 76.72\tiny(.94)  & 84.00\tiny(.34)  & 76.39\tiny(1.18)  & 82.55\tiny(1.15)  \\
\midrule
EDA & 74.74\tiny(1.08) & 81.84\tiny(.59) & 62.04\tiny(2.49) & 66.78\tiny(1.53) & 75.88\tiny(1.59)  & 81.91\tiny(.67)  & 77.17\tiny(1.85)  & 83.12\tiny(1.30)  \\
BT & 75.12\tiny(1.03) & 84.12\tiny(.28) & 60.83\tiny(1.16)  & 68.34\tiny(1.33) & 77.31\tiny(.72)  & 82.89\tiny(.21)  & 77.49\tiny(2.71)  & 82.05\tiny(1.45)  \\
PrompDA & 70.36\tiny(1.85) & 78.85\tiny(1.56) & 58.08\tiny(4.98)  & 64.56\tiny(3.64) & 69.86\tiny(4.27)  & 74.87\tiny(3.02)  & 70.80\tiny(3.16)  & 78.60\tiny(1.49)  \\
SuperGen & 70.36\tiny(1.85) & 78.85\tiny(1.56) & 58.08\tiny(4.98)  & 64.56\tiny(3.64) & 69.86\tiny(4.27)  & 74.87\tiny(3.02)  & 70.80\tiny(3.16)  & 78.60\tiny(1.49)  \\
GPT-J & 76.58\tiny(1.30) & 83.01\tiny(.87) & 62.16\tiny(1.83) & 71.45\tiny(1.86) & 76.59\tiny(.94) & 81.65\tiny(.73)   & 77.91\tiny(2.22) & 82.51\tiny(1.90)  \\
\midrule
CA & \textbf{78.74\tiny{(1.00)}} & \textbf{85.95\tiny{(.34)}} & \textbf{63.17\tiny{(2.20)}} & \textbf{71.30\tiny{(1.54)}} &  \textbf{79.02\tiny{(.89)}} &  \textbf{85.49\tiny{(.35)}} & 76.51\tiny{(2.77)} & \textbf{83.98\tiny{1.17)}} \\
\bottomrule
\end{tabular}
\caption{BERT-based evaluation results.}
\label{table: table: analysis_context_aug_versus_data_aug_full: subtable, roberta}
\end{subtable}
\caption{Comparison of contextual augmentation against data augmentation. CA denotes contextual augmentation. The top results are highlighted.}
\label{table: analysis_context_aug_versus_data_aug_full}
\end{table*}

==> latex_tables/analysis_context_aug_versus_data_aug_full_bert.tex <==
\begin{table*}[t]
%% local redefinitions
% \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
% \renewrobustcmd{\boldmath}{}
\centering
\small
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & 
\multicolumn{2}{c}{BANKING77} &
\multicolumn{2}{c}{HINT3} &
\multicolumn{2}{c}{HWU64} &
\multicolumn{2}{c}{MCID}  
\\
\cmidrule(lr){2-3}  \cmidrule(lr){4-5}  \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& 5-shot & 10-shot & 5-shot & 10-shot & 5-shot & 10-shot & 5-shot & 10-shot\\
\midrule
% ChildTune & xx & xx & xx  & xx & xx  & xx  & xx  & xx  \\
% NoisyTune & xx & xx & xx  & xx & xx  & xx  & xx  & xx  \\
DFT & 69.01\tiny(1.54) & 78.92\tiny(1.69) &  60.65\tiny(1.60)  & 66.36\tiny(3.48) & 75.07\tiny(.53)  & 82.38\tiny(1.49)  & 72.32\tiny(1.80)  & 80.53\tiny(1.15)  \\
\midrule
EDA & 68.81\tiny(1.97) & 72.97\tiny(.94) & 60.50\tiny(3.06) & 59.94\tiny(1.10) & 74.68\tiny(.81)  & 72.76\tiny(5.16)  & 73.10\tiny(.64)  & 80.99\tiny(.16)  \\
BT & 69.65\tiny(1.39) & 78.42\tiny(.83) & 60.50\tiny(1.40)  & 66.33\tiny(2.69) & 74.15\tiny(.84)  & 79.12\tiny(1.65)  & 75.15\tiny(2.04)  & 81.36\tiny(1.6)  \\
PrompDA & 70.36\tiny(1.85) & 78.85\tiny(1.56) & 58.08\tiny(4.98)  & 64.56\tiny(3.64) & 69.86\tiny(4.27)  & 74.87\tiny(3.02)  & 70.80\tiny(3.16)  & 78.60\tiny(1.49)  \\
SuperGen & 70.36\tiny(1.85) & 78.85\tiny(1.56) & 58.08\tiny(4.98)  & 64.56\tiny(3.64) & 69.86\tiny(4.27)  & 74.87\tiny(3.02)  & 70.80\tiny(3.16)  & 78.60\tiny(1.49)  \\
GPT-J & 71.84\tiny(1.41) & 78.34\tiny(.87) & 60.24\tiny(.83) & 67.40\tiny(2.41) & 70.72\tiny(.78) & 76.66\tiny(1.3)   & 73.92\tiny(2.77) & 78.77\tiny(2.39)  \\
\midrule
CA & \textbf{72.23\tiny{(1.80)}} & \textbf{82.33\tiny{(.72)}} & 60.53\tiny{(2.73)} & \textbf{70.36\tiny{(1.90)}} &  76.73\tiny{(1.05)} & 82.61\tiny{(.23)} & 77.45\tiny{(1.66)} & 81.27\tiny{(1.41)} \\
\bottomrule
\end{tabular}
\caption{Comparison of contextual augmentation against data augmentation. CA denotes contextual augmentation. The best results are highlighted.}
\label{table: table: analysis_context_aug_versus_data_aug_full: subtable, bert}
\label{table: analysis_context_aug_versus_data_aug_full}
\end{table*}

==> latex_tables/experiment_DFT_best_hyper_parameter.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{lp{5.5cm}}
\toprule
PLM   &  Hyper-parameter \\
\midrule
BERT      &  $\text{lr}_\text{PLM}=2e-4$, $\text{lr}_\text{cls}=2e-5$, $\lambda=1.0$, context\_size =50, $t=100$, $\text{iteration}$=6.  \\
\midrule
RoBERTa   &  $\text{lr}_\text{PLM}=2e-5$, $\text{lr}_\text{cls}=2e-3$, $\lambda=0.1$, context\_size =50, $t=40$,  $\text{iteration}$=5. \\
\bottomrule
\end{tabular}
\caption{Hyper-parameters of DFT. $\text{lr}_\text{PLM}$ and $\text{lr}_\text{cls}$ denote the learning rate of the PLM and the linear classifier, respectively. context\_size is the size of the augmented context utterances per label. iteration is the iteration of sequential self-distillation.}
\label{table: DFT_details_best_hyper-parameters}
\end{table}

==> latex_tables/experiment_DFT_grid_search_range.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{lp{4.5cm}}
\toprule
Parameter &  Range \\
\midrule
$\text{lr}_\text{PLM}$ & $\{2e-5, 2e-4, 2e-3\}$ \\
$\text{lr}_\text{cls}$ & $\{2e-5, 2e-4, 2e-3\}$ \\
\bottomrule
\end{tabular}
\caption{Grid search range of hyper-parameters for DFT and IntentBERT.}
\label{table: DFT_details_hyper-parameters_range}
\end{table}
